Aggregated Momentum: Stability Through Passive Damping

Momentum is a simple and widely used trick which allows gradient-based optimizers to pick up speed along low curvature directions. Its performance depends crucially on a damping coefficient $\beta$. Large $\beta$ values can potentially deliver much larger speedups, but are prone to oscillations and instability; hence one typically resorts to small values such as 0.5 or 0.9. We propose Aggregated Momentum (AggMo), a variant of momentum which combines multiple velocity vectors with different $\beta$ parameters. AggMo is trivial to implement, but significantly dampens oscillations, enabling it to remain stable even for aggressive $\beta$ values such as 0.999. We reinterpret Nesterov's accelerated gradient descent as a special case of AggMo and analyze rates of convergence for quadratic objectives. Empirically, we find that AggMo is a suitable drop-in replacement for other momentum methods, and frequently delivers faster convergence.

==> evaluation/eval_funnel.tex <==
\subsection{Gaussian Funnels}\label{sec:gaussian_funnel}

In order to demonstrate that AggMo kills off oscillations and improves convergence in practice, we compare CM, Nesterov and AggMo on a realistic 1D regression problem. We randomly sample 1000 points from a standard normal distribution, and compute the function value $y_i = \begin{cases} 0.5 \sin(3 x_i), & \text{if $-1 \le x_i \le 1$}\\ 0.5 \sin(3)x_i, & \text{otherwise} \end{cases}+ \epsilon_i, \epsilon_i \sim \mathcal{N}(0, 0.02)$.
We use a two-hidden-layer Relu network with 10 hidden units to fit the function while setting model observation noise stddev as true value $0.02$. To train the network, we minimize minus the training log likelihood. Because of the small stddev, the surface of the log-likelihood around the optimum is very sharp. Therefore this setting resembles classical funnel problems which is inclined to oscillating.

We use damping vectors $[0, 0.9, 0.99, 0.999]$ for AggMo and $0.999$ for CM as well as Nesterov. The learning rate is tuned over $\{1\mathrm{e-}6, 2\mathrm{e-}6, 3\mathrm{e-}6\}$. We train them all for $4000$ iterations and plot the training loss using log scale in Fig~\ref{fig:1d_regression}. As observed, CM oscillates heavily in this funnel problem and cannot converge to the optimum. AggMo and Nesterov kills off oscillations better and show faster convergence. In particular, AggMo shows almost no oscillations and converges consistently, while Nesterov still suffers from oscillations.

\begin{figure*}
    \vspace{-0.2cm}
    \begin{center}
            \includegraphics[width=0.8\linewidth]{imgs/1D_regression_logscale.png}
        \caption{\textbf{Fitting 1D Regression.} We plot training loss when training a neural network for fitting a funnel 1D regression problem.}\label{fig:1d_regression}
    \end{center}
    \vspace{-0.2cm}
\end{figure*}%

